Q-Pensieve: Boosting Sample Efficiency of Multi-Objective RL Through Memory Sharing of Q-Snapshots

Many real-world continuous control problems are in the dilemma of weighing the pros and cons, multi-objective reinforcement learning (MORL) serves as a generic framework of learning control policies for different preferences over objectives. However, the existing MORL methods either rely on multiple passes of explicit search for finding the Pareto front and therefore are not sample-efficient, or utilizes a shared policy network for coarse knowledge sharing among policies. To boost the sample efficiency of MORL, we propose Q-Pensieve, a policy improvement scheme that stores a collection of Q-snapshots to jointly determine the policy update direction and thereby enables data sharing at the policy level. We show that Q-Pensieve can be naturally integrated with soft policy iteration with convergence guarantee. To substantiate this concept, we propose the technique of Q replay buffer, which stores the learned Q-networks from the past iterations, and arrive at a practical actor-critic implementation. Through extensive experiments and an ablation study, we demonstrate that with much fewer samples, the proposed algorithm can outperform the benchmark MORL methods on a variety of MORL benchmark tasks.

==> 4-analysis.tex <==




==> table_temp.tex <==



\begin{table*}[!htb]
    \centering
    % \setlength{\tabcolsep}{} %% default is 6pt
    \caption{Comparison of MOSAC and other baseline algorithms in three metrics across six experimental domains. Each result is conducted over five random seeds. Each seed is performed in 100 preferences, and each preference is performed 20 times. And the EPD is calculated by comparing to Vanilla MOSAC (MOSAC without Q-Committee assistance).}
    \label{tab:expResult}
    \begin{tabular}{l c c c c c c}
         \hline Environments & Metrics & PFA & PGMORL & CN-DER  & \textbf{Q-Committee} \\
         \hline
         \hline
          & HV($\times 10^2$)& 8.6$\pm$1.3 & 8.2$\pm$1.5 & 5.36  & \textbf{10.21}\\
         \cline{2-6}
         DST & UT &-6.0$\pm$6.8 & 4.3$\pm$2.0 & -5.10 & \textbf{7.31}\\
         \cline{2-6}
          & EPD & 0.11$\pm$0.09 & 0.27$\pm$0.21 & 0.21 & \textbf{0.54}\\
         \hline
         & HV($\times 10^7$)& - & 19.3$\pm$8.6 & 15.3$\pm$6.1 & \textbf{20.5$\pm$0.5}\\
         \cline{2-6}
         LunarLander & UT &- & -22.4$\pm$5.0 & 35.7$\pm$29.4 & \textbf{51.4$\pm$1.5}\\
         \cline{2-6}
          & EPD & - &  & 0.21 & \textbf{0.54}\\
         \hline
          & HV($\times 10^6$)& 13.2$\pm$2.6 & 2.8$\pm$2.9 & 20.8$\pm$5.2 & \textbf{38.2$\pm$2.7}\\
         \cline{2-6}
         HalfCheetah & UT & 1016.2$\pm$402.8 & 85.6$\pm$165.8 & 5086.5$\pm$3570.3 &  \textbf{5614.5$\pm$309.0}\\
         \cline{2-6}
          & EPD & 0.10$\pm$0.06 & 0.11$\pm$0.05 &  0.02 & \textbf{0.54}\\
         \hline
          & HV($\times 10^5$)& 10.1$\pm$6.2 & 13.1$\pm$4.8 & 5.60$\pm$1.6 & \textbf{13.3$\pm$2.0}\\
         \cline{2-6}
         Hopper & UT & 349.6$\pm$186.0 & 369.6$\pm$178.5 & 142.6$\pm$98.2 & \textbf{408.0$\pm$110.0}\\
         \cline{2-6}
          & EPD & 0.41$\pm$0.10 & 0.31$\pm$0.11 & 0.04 & \textbf{0.43}\\
         \hline
          & HV($\times 10^8$)& - & 9.1$\pm$13.92 & 36.68 & \textbf{95.6$\pm$6.0}\\
         \cline{2-6}
         Hopper3d & UT & - & 312.7$\pm$261.7 & 724.37 & \textbf{1393.9$\pm$147.0}\\
         \cline{2-6}
          & EPD & - & 0.03$\pm$0.03 & 0.07 & \textbf{0.55}\\
         \hline
          & HV($\times 10^4$)& 77.3$\pm$53.4 & 13.4$\pm$4.2 & 501.59$\pm$359.7 & \textbf{1000.7$\pm$186.0}\\
         \cline{2-6}
         Ant & UT & 11.7$\pm$13.8 & -18.9$\pm$38.2 & 367.60$\pm$234.1 & \textbf{1403.8$\pm$303.0} \\
         \cline{2-6}
          & EPD & 0.22$\pm$0.02 & 0.21$\pm$0.03 & 0.21 &\textbf{0.60}\\
         \hline
         & HV($\times 10^7$)& - & 6.5$\pm$5.5 & 130.0$\pm$41.1 & \textbf{218.7$\pm$ 10.7}\\
         \cline{2-6}
         Ant3d & UT & - & 252.6$\pm$35.3 & 487.8$\pm$234.4 & \textbf{1138.1$\pm$227.3} \\
         \cline{2-6}
          & EPD & - &  & 0.21 &\textbf{0.60}\\
         \hline
          & HV($\times 10^5$)& 10.5$\pm$4.4 & \textbf{12.8$\pm$6.6} & 4.21 & 11.2$\pm$3.6 \\
         \cline{2-6}
         Walker2d & UT & 95.5$\pm$54.6 & 280.3$\pm$327.6 & 317.58 & \textbf{637.5$\pm$142.0}\\
         \cline{2-6}
          & EPD & 0.10$\pm$0.10 & 0.16$\pm$0.17 & 0.21 & \textbf{0.48}\\
         \hline
    \end{tabular}
\end{table*}

\begin{table}[]
\begin{tabular}{ccccccc}
Environments & Metrics & \multicolumn{1}{l}{1 pref} & 2 pref & 2 pref with buf & 4 pref & 4 pref with buf \\ \hline
\multirow{3}{*}{HalfCheetah} & HV($\times 10^6$) & 38.30    & 37.76   & 37.20   & 38.91   & 38.20   \\ \cline{2-7} 
                             & UT                & 5477.64 & 5502.26 & 5456.99 & 5673.21 & 5614.52 \\ \cline{2-7} 
                             & EPD               & -       & 0.51    & 0.47    & 0.49    & 0.54    \\ \hline
\multirow{3}{*}{Hopper}      & HV($\times 10^5$) & 11.83   & 10.52   & 12.74   & 11.03   & 14.36   \\ \cline{2-7} 
                             & UT                & 386.47  & 368.15  & 374.23  & 417.29  & 408     \\ \cline{2-7} 
                             & EPD               & -       & 0.45    & 0.51    & 0.48    & 0.43    \\ \hline
\multirow{3}{*}{Hopper3d}    & HV($\times 10^8$) & 61.92   & 63.15   & 69.35   & 75.14   & 78.34   \\ \cline{2-7} 
                             & UT                & 1521.06 & 1662.15 & 1734.35 & 1762.34 & 1742.91 \\ \cline{2-7} 
                             & EPD               & -       & 0.47    & 0.50    & 0.52    & 0.55    \\ \hline
\multirow{3}{*}{Ant}         & HV($\times 10^5$) & 85.22  & 84.16  & 87.43  & 94.37  & 100.07 \\ \cline{2-7} 
                             & UT                & 940.53  & 973.62  & 1005.25 & 1211.51 & 1252.84 \\ \cline{2-7} 
                             & EPD               & -       & 0.51    & 0.50    & 0.55    & 0.60    \\ \hline
\multirow{3}{*}{Walker2d}    & HV($\times 10^5$) & 14.32   & 9.24    & 11.88   & 10.95   & 12.04   \\ \cline{2-7} 
                             & UT                & 513.32  & 517.27  & 550.75  & 617.75  & 637.48  \\ \cline{2-7} 
                             & EPD               & -       & 0.50    & 0.48    & 0.51    & 0.48    \\ \hline
\end{tabular}
\end{table}
